On Completeness of Logical Relations for Monadic Types

Software security can be ensured by specifying and verifying security properties of software using formal methods with strong theoretical bases. In particular, programs can be modeled in the framework of lambda-calculi, and interesting properties can be expressed formally by contextual equivalence (a.k.a. observational equivalence). Furthermore, imperative features, which exist in most real-life software, can be nicely expressed in the so-called computational lambda-calculus. Contextual equivalence is difficult to prove directly, but we can often use logical relations as a tool to establish it in lambda-calculi. We have already defined logical relations for the computational lambda-calculus in previous work. We devote this paper to the study of their completeness w.r.t. contextual equivalence in the computational lambda-calculus.

==> conclu.tex <==
\section{Conclusion}
\label{sec:conclusion}

The work presented in this paper is a natural continuation of the
authors' previous work \cite{GLLN02,GLLNZ04}. In \cite{GLLN02}, we
extend \cite{MS93-sconing} and derive logical relations for monadic
types which are sound in the sense that the Basic Lemma still
holds. In \cite{GLLNZ04}, we study contextual equivalence in a
specific version of the computational $\lambda$-calculus with
cryptographic primitives and we show that lax logical relations (the
categorical generalization of logical relations \cite{lax-lr})
derived using the same construction is complete.  Then in this paper,
we explore the completeness of logical relations for the
computational $\lambda$-calculus and we show that they are complete at
first-order types, for a list of common monads: partial computations,
exceptions, state transformers and continuations, while in the case of 
continuation, the completeness depends on a natural constant $\ccall{}{}$, 
with which we cannot show the soundness.


Pitts and Stark have defined operationally based logical relations to
characterize the contextual equivalence in a language with local store
\cite{PS98-equiv-state}.  This work can be traced back to their early
work on the nu-calculus \cite{PS93-new} which can be translated in a
special version of the computational $\lambda$-calculus and be modeled
using the dynamic name creation monad \cite{Stark96-new-model}.
%However this monad is not defined of the category $\catset$.
Logical relations for this monad are derived in
\cite{Zhang-thesis} using the construction from \cite{GLLN02}.  It is
also shown in \cite{Zhang-thesis} that such derived logical relations
are equivalent to Pitts and Stark's operational logical relations up
to second-order types.

An exceptional case of our completeness result is the non-determinism
monad, where logical relations are not complete for all first-order
types, but a subset of them.  We effectively show this by providing a
counter-example that breaks the completeness at first-order
types. This is indeed an interesting case. A more comprehensive study
on this monad can be found in \cite{Jeffrey99-nondetermin-monad},
where Jeffrey defines a denotational model for the computational
$\lambda$-calculus specialized in non-determinism and proves that this
model is fully abstract for may-testing. The relation between our
notion of contextual equivalence and the may-testing equivalence
remains to be clarified.

%We were expecting to find a general proof for completeness of logical
%relations for monadic types, perhaps with some restrictions on monads
%or types.  We follow in particular the categorical construction
%defined in \cite{GLLN02}.

Recently, Lindley and Stark introduce the syntactic $\top\top$-lifting
for the computational $\lambda$-calculus and prove the strong
normalization \cite{Stark05:TT-lifting}. Katsumata then instantiates
their liftings in $\catset$ \cite{Katsumata05:TT-lifting-set}.  
The $\top\top$-lifting of strong monads
is an essentially different approach from that in \cite{GLLN02}. It
would be interesting to establish a formal relationship between these
two approaches, and to look for a general proof of completeness using
the $\top\top$-lifting.

%% \subsubsection{Acknowledgement}

%% The authors are grateful to anonymous reviewers for their comments on earlier versions,
%% which help the authors to improve the paper.


==> intro.tex <==
\section{Introduction}

\subsubsection*{Contextual equivalence.}
Two programs are contextually equivalent (a.k.a.\ observationally equivalent) if they 
have the same observable behavior, i.e. an outsider cannot distinguish them.
Interesting properties of programs can be expressed using the notion of contextual
equivalence.
%
For example, to prove that a program does not leak a secret, such as the secret key used 
by an ATM to communicate with the bank, it is sufficient to prove that if we change the 
secret, the observable behavior will not change 
\cite{SP-lr,GLLNZ04,Zhang-thesis}: 
whatever experiment a customer makes with the ATM, he or she cannot guess information 
about the secret key by observing the reaction of the ATM.
%
Another example is to specify functional properties by contextual equivalence. For example, 
if $\mbox{\small\sf sorted}$ is a function which checks that a list is sorted and 
$\mbox{\small\sf sort}$ is a function which sorts a list, then, for all list $l$, you want 
the expression $\mbox{\small\sf sorted}(\mbox{\small\sf sort}(l))$ to be contextually 
equivalent to the expression $\mbox{\small\sf true}$.
Finally, in the context of parameterized verification, contextual equivalence allows the 
verification for all instantiations of the parameter to be reduced to the verification 
for a finite number of instantiations (See e.g.\ \cite{LN00} where logical relations are 
one of the essential ingredients).

\subsubsection*{Logical relations.}
While contextual equivalence is difficult to prove directly because of the universal 
quantification over contexts, logical relations \cite{Plotkin80,Mitchell96} 
% and pre-logical relations \cite{prelogrel} 
are powerful tools that allow us to deduce contextual equivalence in typed $\lambda$-calculi.
With the aid of the so-called Basic Lemma, one can easily prove that logical relations 
are sound w.r.t.\ contextual equivalence. However, completeness of logical relations 
is much more difficult to achieve:
%whereas pre-logical relations are complete at all types,
usually we can only show the completeness of logical relations  for types up to first order.

\iflong
On the other hand, the computational $\lambda$-calculus \cite{Moggi91} has proved useful 
to define various notions of computations on top of the $\lambda$-calculus: partial 
computations, exceptions, state transformers, continuations and non-determinism in particular.
Moggi's insight is based on categorical semantics: while categorical models 
of the standard $\lambda$-calculus are cartesian closed categories (CCCs), 
the computational $\lambda$-calculus requires CCCs with a strong monad.
%% According to Moggi, a faithful categorical model for the computational $\lambda$-calculus 
%% must be a cartesian closed category (CCC) equipped with a strong monad. 
Logical relations for monadic types, which are particularly introduced in Moggi's language, 
can be derived by the construction defined in \cite{GLLN02} where soundness of 
logical relations is guaranteed.

\else
The computational $\lambda$-calculus \cite{Moggi91} has proved useful to define 
various notions of computations on top of the $\lambda$-calculus, using monadic types. 
Logical relations for \linebreak monadic types can be derived by the 
construction defined in \cite{GLLN02} where soundness of logical relations is guaranteed.
\fi
%
However, monadic types introduce new difficulties. In particular, contextual equivalence 
becomes subtler due to the different semantics of different monads: equivalent programs 
in one monad are not necessarily equivalent in another! This accordingly makes completeness 
of logical relations more difficult to achieve in the computational $\lambda$-calculus. 
In particular the usual proofs of completeness up to first order do not go through. 

\iflong
\else
\vspace*{-1.6em}
\fi

\subsubsection*{Contributions.}
We propose in this paper a notion of contextual equivalence for the computational 
$\lambda$-calculus. Logical relations 
%and pre-logical relations
for this language are defined according to the general derivation in \cite{GLLN02}.
We then explore the completeness and we prove that for the partial computation monad, 
the exception monad and the state transformer monad, logical relations are still 
complete up to first-order types. In the case of the non-determinism monad, we need 
to restrict ourselves to a subset of first-order types. 
\iflong
As a corollary, we prove that strong bisimulation is complete w.r.t.\ contextual 
equivalence in a $\lambda$-calculus with monadic non-determinism.
\else
\fi

Not like previous work on using logical relations to study contextual equivalence 
in models with computational effects 
\cite{Sieber96,PS98-equiv-state,OHearnTennent95},
% \else
% \cite{PS98-equiv-state},
% \fi
most of which focus on computations with local states,
our work in this paper is based on a more general framework for describing computations,
namely the computational $\lambda$-calculus. In particular, very different forms of 
computations 
\iflong
like continuations and non-determinism are studied, 
\else 
like non-determinism are studied,
\fi
not just those for local states.

\iflong
\subsubsection*{Plan.}
The rest of this paper is structured as follows:
we devote Section~\ref{sec:simpcal} to preliminaries, by introducing basic knowledge 
of logical relations in a simple version of typed $\lambda$-calculus;
then from Section~\ref{sec:compcal} on, we move to the computational $\lambda$-calculus
and we rest on a set-theoretical model. In particular, Section~\ref{sec:compcal.general-proof} 
sketches out the proof scheme of completeness of logical relations for monadic types 
and shows the difficulty of getting a general proof; we then switch to case studies 
and we explore, in Section~\ref{sec:complete}, the completeness 
in the computational $\lambda$-calculus for a list of common monads:
partial computations, exceptions, state transformers, continuations and the non-determinism;
the last section consists of a discussion on related work and perspectives. 
\else
Note that all proofs that are omitted in this short paper, 
can be found in the full version \cite{LNZ-complete-long}.
\fi


==> macros.tex <==
\newcommand{\lamarrow}{\lambda^{\to}}
\newcommand{\lamcomp}{\lambda_{\mathit{Comp}}}
\iflong
\newcommand{\sublamcomp}{\lambda_{\mathit{Comp}}^{\mathit{PESCN}}}
\newcommand{\subsublamcomp}{\lambda_{\mathit{Comp}}^{\mathit{PESC}}}
\else
\newcommand{\sublamcomp}{\lambda_{\mathit{Comp}}^{\mathit{PESN}}}
\newcommand{\subsublamcomp}{\lambda_{\mathit{Comp}}^{\mathit{PES}}}
\fi

\newcommand{\compreduc}{\beta c}

\newcommand{\Eval}[1]{{\left\llbracket{#1}\right\rrbracket}}
\newcommand{\leval}{\llbracket}
\newcommand{\reval}{\rrbracket}

\newcommand{\ord}[1]{\mathbf{ord}({#1})}
\newcommand{\jud}[3]{{#1} \vdash {#2} {\ : \ } {#3}}
\newcommand{\arr}[2]{{#1}\to{#2}}
\newcommand{\obs}{\mathbf{Obs}}
%% \newcommand{\set}{\mathrm{Set}}
\newcommand{\set}[1]{\{#1\}}
%% \newcommand{\rel}{\mathrm{Rel}}
\newcommand{\liftt}{\tilde{T}}
\newcommand{\defi}[1]{\mathsf{def}_{#1}}
\newcommand{\deffi}[1]{\mathsf{def}^2_{#1}}
\newcommand{\fp}[1]{{\mathbb{P}}_\mathrm{fin}(#1)}
\newcommand{\cpair}[1]{\langle{#1}\rangle}
\newcommand{\metafun}{\underline{\lambda}\,}
\newcommand{\compdeg}{\delta}

\newcommand{\Kc}{\mathtt{K}}
\newcommand{\Sc}{\mathtt{S}}
\newcommand{\val}[1]{{\tt val(}{#1}{\tt )}}
\newcommand{\letlet}[3]{{\tt let\ }{#1}{\tt \ \Leftarrow \ }{#2}{\tt \ in \ }{#3}}
\newcommand{\cval}{\mathtt{val}}
\newcommand{\clet}[3]{{\tt let\ }{#1}{\tt \ \Leftarrow \ }{#2}{\tt \ in \ }{#3}}
\newcommand{\diver}[1]{{\Omega}^{#1}}
\newcommand{\cunit}{\ast}
\newcommand{\cchoose}[3]{{#2} +_{#1} {#3}}
\newcommand{\cempty}{\Phi}
\newcommand{\ctest}[1]{\mathtt{test}_{#1}}
\newcommand{\craise}[1]{\mathtt{raise}_{#1}}
\newcommand{\ccatch}[3]{\mathtt{catch}\;{#1}\;\mathtt{in}\;{#2}\mathtt{then}\;{#3}}
\newcommand{\ctrue}{\mathtt{true}}
\newcommand{\cfalse}{\mathtt{false}}
\newcommand{\cdoat}[2]{\mathtt{do}\;{#1}\;\mathtt{at}\;{#2}}
\newcommand{\cupdate}[1]{\mathtt{update}_{{#1}}}
\newcommand{\ccall}[2]{\mathtt{call}^{#1}_{#2}}
\newcommand{\ceq}[1]{\mathtt{eq}_{#1}}

\newcommand{\tbool}{\mathsf{bool}}
\newcommand{\tunit}{\mathsf{unit}}
\newcommand{\tcomp}{\mathsf{T}}
\newcommand{\tstate}{\mathsf{state}}
\newcommand{\tlabel}{\mathsf{label}}

\newcommand{\bottom}{\bot}
\newcommand{\state}{\mathit{St}}
\newcommand{\st}{\mathit{St}}
\newcommand{\subst}[3]{{#1}[{#3}/{#2}]}
\newcommand{\med}[2]{{\mathbb d}_{{#1},{#2}}}

\newcommand{\weaktype}[1]{{#1}_\mathrm{w}}
\newcommand{\strongtype}[1]{{#1}_\mathrm{s}}

\newcommand{\identity}{\mbox{id}}
\newcommand{\monadtype}{\mathsf{T}}
\newcommand{\monad}{\mathbf{T}}
\newcommand{\unit}{\eta}
\newcommand{\mult}{\mu}
\newcommand{\strength}{\mathrm{t}}
\newcommand{\setcat}{\mbox{\bf Set}}
\newcommand{\catset}{\mathcal{S}et}

\newcommand{\ce}{\approx}
\newcommand{\ced}{\sim}
\newcommand{\logrel}{(\mathcal{R}_\tau)_{\tau\;\mathrm{type}}}
\newcommand{\rel}{\mathcal{R}}
\newcommand{\lr}[1]{\; \mathcal{R}_{{#1}} \;}
\newcommand{\ilr}[2]{\mathcal{R}_{#1}^{#2}}
\newcommand{\predic}{\mathcal{P}}
\newcommand{\predef}[1]{\mathcal{P}^{\mathsf{def}}_{#1}}
\newcommand{\pcons}{\mathbf{Cond}}

\newcommand{\byzy}[1]{\begin{center}\fbox{\parbox{30em}{\em {\bf ZY:} {#1}}}\end{center}}

\newcommand{\context}{\mathbb{C}}

\newcommand{\cancelled}[1]{}

\newcommand{\settoi}{{\catset}^\mathcal{I}}
\newcommand{\ordinalcat}{\mathcal{I}}
\newcommand{\cati}{\mathcal{I}}
\newcommand{\cnew}{\mathtt{new}}
\newcommand{\tname}{\mathsf{name}}
\newcommand{\minl}{\mathbf{inl}}
\newcommand{\minr}{\mathbf{inr}}
\newcommand{\picat}{{\mathcal{PI}^{\to}}}

